Principle of Need-to-Act

In this paper, we have introduced the notion of "Principle of Need-to- Act". This principle is essential towards developing secure systems, security solutions and analyzing security of a solution.

==> prelim.tex <==
{\em Trees and Graphs}: A directed 
%(a  directed 
graph \graphve\ is a
set of nodes (or vertices) \vset\ and a set of edges \eset\ between these nodes:
\edge{\x}{\y}\ is an edge from \x\ to \y, (\x, \y) \iin\ \vset\ $\times$ \vset.
A node \x\ represents an atomic unit of data, which is always shared as a whole
or is not shared at all. A node \x\ is called the ancestor of a node \y\ iff
there exists a path consisting of one or more edges from \x\ to \y. Node \x\ is
an immediate ancestor of \y\ in \graph\ iff there exists an edge \edge{\x}{\y} in
\eset. Nodes having a common immediate ancestor are called siblings. If there is
a specific order between siblings in \graph, then \graph\ is  an ordered graph.
 The fact that \x\ precedes one of its
siblings \y\ in an ordered graph is denoted by \x\ \precedes\ \y; i.e., \x\ is to
the left of \y. The contents, if any, of a node \x\ is referred to as
\content{\x}. A {\em redacted subgraph} 
 graph \graphve\ is denoted by \subgraphve, and
\subgraphve\ $\subseteq$ \graphve. \subgraphve\ $\subseteq$ \graphve\ if and
only if \vsubset\  $\subseteq$ \vset\ and \esubset\ $\subseteq$ \eset. \subgraphve\ $\subset$ \graphve\ if and
only if \vsubset\ $\cup$ \esubset\ $\subset$ \vset\ $\cup$
\eset. Redacted
subgraph \subgraphve\ is derived from the graph \graphve\ by redacting the set of nodes \vset\ \textbackslash\ \vsubset\ and the set of edges \eset\ \textbackslash\ \esubset\
from  \graph. A directed tree \treeve\ is a
directed graph with the following constraint: removal of any edge \edge{\x}{\y}\ from \eset\ leads to
two disconnected trees  with no edge or path between nodes \x\ and \y. Two
nodes are siblings, if they have a common parent; \x\ is  a parent of  node
\y\ iff  there is an edge \edge{\x}{\y}\ in  \tree; \y\ is called the child of
its parent \x. In a tree, a parent node is nothing but the immediate ancestor
of all its child nodes. An ordered tree is one where each pair of siblings have
an order between them. A rooted tree has a special node called root, for which
there is no parent node. As in the case of graphs, a redacted subtree of tree
\treeve\ is denoted by \subtreeve\ such that \subtreeve\ $\subseteq$ \treeve. \subtreeve\ $\subseteq$ \treeve\ denotes
that \vsubset\  $\subseteq$ \vset\ and \esubset\ $\subseteq$ \eset. Redacted
subgraph \subtreeve\ is derived from the tree \treeve\ by redacting the set
of nodes \vset\ \textbackslash\ \vsubset\ and the set of edges \eset\ \textbackslash\ \esubset\
from  \tree. Two trees/graphs/forests with the same nodes and edges, but
{\em different ordering} between at least one pair of siblings are different
trees/graphs/forests.  
 In the rest of the paper, a tree refers to an ordered directed rooted tree,
 and a graph refers to an ordered directed graph, a subtree/subgraph refers to
 a redacted subtree/subgraph of a tree/graph unless otherwise stated.
 \treegraphve\ refers to either a tree \treeve\ or a graph \graphve. 
% We use $n$ to
% denote the number of nodes in $T$.
% The parent of a node  $v$ is denoted by $\parent{v}$.

==> related.tex <==
Merkle ~\cite{merkle,merklephd}  
proposed a  digital signature scheme based on a secure conventional encryption 
function over a hierarchy (tree) of document fragments. 
Since then,
this technique has been used widely, but always with an authentication path 
of logarithmic size  to verify even a single document fragment. 
There have been several works~\cite{Berman200726,
mht:traversal:optimal:lipmaa02, mht:traversal:jakobsson03} in order to optimize
traversal of Merkle hash trees so that the auxiliary information required for
authentication can be determined efficiently. Improved (more efficient) versions
of MHT have also been proposed~\cite{improved}.

The MHT has been widely used for data
authentication~\cite{mht:uddi:elisa04,mht:wormseal:li:09,uncertain:mht:singh:edbt08,devanbu1,
Devanbu03authenticdata,dbauth-pang-text,haber:signature:asiaccs08}. Bertino {\em et al}.~\cite{bertino-xml} proposed a technique based on the Merkle hash technique for selective dissemination of XML data in a third party distribution
framework. However, there has been no work that has looked into the device data
authentication in an efficient manner.

In \cite{mht:uddi:elisa04}, Bertino {\em et al}. have defined an
authentication scheme using MHT for UDDI repositories towards building  secure
web services directories. Using techniques from incremental cryptography, Naor and
Nissim~\cite{cert:naor:1996} dynamize hash trees to support the insertion and deletion of elements. In their scheme, the source and the directory maintain
identically implemented $2-3$ trees. Each leaf of such a $2-3$  tree  stores an
element of set, and each internal node stores a one-way hash of its children's
values. Hence the source-to-directory communication is reduced to $O(1)$ items,
but the directory-to-user communication remains at $O(log n)$. Thus, their
solution is however not size oblivious.
 Martel {\em et al}.~\cite{martel04}  proposed an
authentication technique for data structures - directed acyclic graphs referred
to as ``Search DAGs'' in third party distribution frameworks. However their
technique uses Merkle hash technique~\cite{merkle}.
Moreover the ``Search DAGs'' technique only covers DAGs, not the general directed graphs. For secure
multicast, Perrig uses static data ordering over symmetric encryption
~\cite{perrig}. Li {\em et al}.~\cite{mht:wormseal:li:09} propose a scheme
for trustworthy verification (authentication) of write-only read-many data
based on the MHT. Singh and Prabhakar~\cite{uncertain:mht:singh:edbt08}
developed an authentication scheme for uncertain databases using MHT.
Kocher ~\cite{kocher} presented a scheme using Merkle hash technique for data
distribution using third party models. 

 Authenticated data structures (ADS's) have been used 
to verify the authenticity of data in a static as well as in the dynamic
context. Goodrich and
Tamassia~\cite{goodrich00efficient} proposed authenticated dictionaries using 
skip lists and commutative hashing (one-way accumulators). Goodrich 
{\em et al.}~\cite{goodrich-graphs} proposed techniques to authenticate graphs with
specific path queries and geometric searching.  
Goodrich {\em et al}.~\cite{goodrich-graphs} define a generalized
Merkle Hash tree for paths in graphs, and propose a mechanism for authenticating
path queries in graphs. They leak structural information
because their notion of ``path hash accumulator'' and 
their use of generalized merkle hash technique.  Martel {\em et
al}. also proposed Search DAGs~\cite{martel04} using the Merkle hash technique. Papamanthou {\em et
al}. ~\cite{papamanthou:authhash:ccs08} propose authenticated hash tables, where
leakage-free property is not achieved, rather efficiency is of primary concern.
Goodrich {\em et al}.~\cite{goodrich-graphs} provides an excellent related works
section on authenticated data structures and we refer interested readers to this
paper. Atallah {\em et al}.~\cite{icde08} have developed a scheme for 
authentication of 2-dimensional data using only one aggregate signature.
Atallah {\em et al}.~\cite{ipl08} developed schemes for covering a tree with minimum
number of paths such that the total number of nodes in all the paths is
minimized. Such a scheme has applications in verification of integrity of trees
and paths. 
